Stochastic Backpropagation and Approximate Inference in Deep Generative Models

We marry ideas from deep neural networks and approximate Bayesian inference to derive a generalised class of deep, directed generative models, endowed with a new algorithm for scalable inference and learning. Our algorithm introduces a recognition model to represent approximate posterior distributions, and that acts as a stochastic encoder of the data. We develop stochastic back-propagation -- rules for back-propagation through stochastic variables -- and use this to develop an algorithm that allows for joint optimisation of the parameters of both the generative and recognition model. We demonstrate on several real-world data sets that the model generates realistic samples, provides accurate imputations of missing data and is a useful tool for high-dimensional data visualisation.

==> 2014_icml_NGBR 2/background.tex <==
\begin{figure}[t]
 \vskip 0.2in
 \begin{center}
 \centerline{\includegraphics[width=\columnwidth]{FIGURE_Intro}}
 \caption{
 The class of generative models studied in this paper.  {\bf (a)} 
 Diagram of our model.  {\bf (b)} Diagram corresponding to 
 the equivalent representation (\ref{eq:LogLike}).
 {\bf (d)}  The computational diagram indicating the connectivity of the 
 generative and recognition models during learning.}
\label{figure:introModel}
\end{center}
\vskip -0.2in
\end{figure} 

In contrast to the Helmholtz machines originally introduced in 
\citep{Dayan1995, Dayan2000} which uses discrete latent variables, we 
have adopted  Gaussian latent variables. 

This choice was motivated by Price's \citep{Price1958} and Bonnet's 
\citep{Bonnet1964} theorems that allow us to interchange the gradients of 
expectations with respect to the moments of a Gaussian distribution with 
the expectation of gradients with respect to the random variables 
\citep{Opper2009}. These properties will be used in the next section to 
compute gradients of the generative and recognition model.

We exploit these nice properties for deriving our learning scheme in the 
following section.

In addition, we would like to model data of different types, i.e. data that 
may be binary, categorical, real-valued, etc. To achieve this objective, we 
make use of the exponential family of distributions, which is an important 
family of distributions that emphasises the shared properties of many 
standard distributions, including the Binomial, Poisson, Gamma, Beta, 
Multinomial, and Gaussian distributions \cite{book:bickel2001}. The 
exponential family of distributions allows us to provide a singular 
discussion of the inferential properties associated with members of the 
family and thus, to develop a modelling framework generalised to all 
members of the family.

In the exponential family of distributions, the conditional probability of 
some observed data vector $\vis$ 
given parameter value $\boldsymbol{\eta}$ takes the following form:
\begin{align}
\label{eq:exponFam}
 p(\vis | \boldsymbol{\eta}) &= \exp \{ s(\vis)^\top \boldsymbol{\eta} 
 + 
 h(\vis) - g(\boldsymbol{\eta}) \},
\end{align}
where $s(\vis)$ are the sufficient statistics, $\boldsymbol{\eta}$ is a 
vector of natural parameters, $h(\vis_n)$ is a function of the data and 
$g(\boldsymbol{\eta})$ is the cumulant or log-partition function. 
For convenience, we shall represent a variable $\vis$ that is drawn from 
an exponential family distribution using the notation: $\vis\sim 
\Expon{\boldsymbol{\eta}}$, with natural parameters 
$\boldsymbol{\eta}$. 

As an example, consider binary data, for which an appropriate data 
distribution is the Bernoulli distribution. The Bernoulli distribution for a 
single component $\vis_i$ has the form: 
$p(\vis_i|\mu) = \mu^{x}(1-\mu)^{1-x}$, with $\mu$ in [0,1]. The 
exponential 
family form, using the terms in Equation (\ref{eq:exponFam}), is described 
using: $h(\vis_i) = 
0$, $\eta = \ln(\frac{\mu}{1 - \mu})$ and $g(\eta) = \ln(1 + e^{\eta})$. 

The natural parameters can be mapped to the parameter values of the 
distribution using the link function, which is the logistic sigmoid in the 
case of the Bernoulli distribution.

More specifically, we are interested in directed generative models 
with a layered structure composed of $L+1$ layers, the $L$th layer being 
the topmost one as shown in Figure~\ref{figure:introModel}{\bf (a)}, 
defined by the equations:

\begin{align}
\hid_{L} &= G_{L} \xi_{L} \label{eq:xL} \\
\hid_{l} &= T_l(\hid_{l+1}) + G_{l} \xi_{l},  \forall l =1 \ldots L-1 
\label{eq:HiddenGen} \\
\vis & \sim  \Expon{T_0(\hid_{1})},
\label{eq:Visible}
\end{align}

where $\hid_{l,i}$ is the vector of activations at layer $l$,
$\xi_{l,j}$ are independent Gaussian random variables with mean 
zero and variance one, $\vis$ is the vector of observed units, 
Bern$(\vec{u})$ is a product of independent 
Bernoulli distributions with probability $p_i=\text{sigmoid}(u_i)$.

Finally $T_l$ are arbitrary maps represented by multi-layer 
perceptrons (MLPs) and $G_l$ are constant matrices. In the 
following we refer to the set of parameters in  $T_l$ and $G_l$  by 
$\theta^g$.

We adopt a weak Gaussian prior over $\theta^g$, $p(\theta^g) = 
\N(\theta| 0, \kappa)$.

This model has a likelihood function of the form

\begin{align}
p(\vis, \hid) &= p(\vis| \hid_1 ) p(\hid_L) p(\theta)
\prod_{l=1}^{L 
- 1} p_l( \hid_l | \hid_{l+1} ),\label{eq:LogLikeStandard} 
\end{align}

where $p( \hid_l | \hid_{l+1} )$ is a distribution implicitly 
defined by equation (\ref{eq:HiddenGen}) and $p(\theta)$ is a prior over 
the model's parameters. The diagram associated to this 
model is shown in Figure \ref{figure:introModel}{\bf (a)}.
 
The conditional distributions
$p_l( \hid_l | \hid_{l+1} )$ are a Gaussian distributions with mean $\mu_l 
= T_l(\hid_{l+1})$ and covariance matrix $S_l = G_l G_l^T$ due to the 
additive property of Gaussians. 

Moreover, when the maps 
$T_l$ are of the form $T_l(\hid) = A_l f(\hid) + b_l $ for some matrix 
$A_l$ and some constant vector $b_l$, 
$G_l$ is a diagonal matrix and $f$ is some 
element-wise non-linearity, Equation (\ref{eq:HiddenGen}) reduces to

\begin{align}
\hid_l &= A_l f(\hid) + b_l + C_l \xi_l,
\end{align}

and we recover the standard non-linear Gaussian belief networks 
\cite{Frey1996, 
Frey1999a}. 

Alternatively, we can interpret the variables $\hid_l$ as deterministic 
functions of the noise variables $\xi_l$.  This can be formally introduced 
as a coordinate transformation of the probability density in Equation 
(\ref{eq:LogLikeStandard}). That is, we perform a change of coordinates $
\hid_l \rightarrow \xi_{l}$. The density of the transformed variables 
$\xi$ can be expressed in terms of the density (\ref{eq:LogLikeStandard}) 
times the Jacobian of the transformation $ p(\xi)  = p(\hid(\xi)) 
|\frac{\partial \hid}{\partial \xi}| $. Since the coordinate transformation is 
linear we have $|\frac{\partial \hid}{\partial \xi}| = |G_l|$ and the density 
of $\xi$ is obtained as follows

\begin{align}
p(\xi) &= p(\hid_L)  |G_L|
\prod_{l=1}^{L - 1}  |G_l| p_l( \hid_l | \hid_{l+1} ) \nonumber  \\
&=  \prod_{l=1}^{L} |G_l| |S_l|^{-\frac{1}{2}}  \N( \xi_l ) \nonumber \\
&=  \prod_{l=1}^{L}  |G_l| |G_l G_l^T|^{-\frac{1}{2}} \N( \xi_l ) \nonumber 
\\
 &= \prod_{l=1}^{L} \N( \xi_l ), 
\end{align}
where $\N(\xi)$ is a Gaussian with mean zero and covariance equal 
to 
the identity matrix. 

Finally the joint density $p(\vis,\xi,\theta)$ can be written as 

\begin{align}
p(\vis,\xi) &= p(\vis| \hid_1( \xi_{1 \ldots L} ) ) p(\theta) 
\prod_{l=1}^{L} 
\N( \xi_l ). \label{eq:LogLike}
\end{align}

The diagram associated to this 
representation is shown in Figure \ref{figure:introModel}{\bf (b)}. 


The likelihood in Equation (\ref{eq:LogLike}) has the interesting property 
that its gradient with respect to $\xi$ backpropagates from the visible 
neurons to the last hidden layer. That is, it takes into account the 
\emph{entire network}. This is to contrast with purely local methods such 
as the wake-sleep and the mean-field algorithms which requires 
several iterations to allow the information to flow from the visible units to 
the top layers.

Moreover, this representation makes it explicit that the generative model 
works by applying a highly non-linear transformation to a spherical 
Gaussian distribution $\N(\xi)$ such that the transformed distribution tries 
to match the empirical distribution.

==> 2014_icml_NGBR 2/conclusion.tex <==
\vspace{-3mm}
\section{Conclusion}
\label{sec:Discussion}

%Our algorithm generalises to a large class of models with continuous latent 
%variables, which include Gaussian, non-negative or sparsity-promoting 
%latent variables. For models with discrete latent variables (e.g., sigmoid 
%belief 
%networks), control variate methods that improve upon the REINFORCE 
%algorithm remain the most general, but intelligent design is needed to 
%control the gradient-variance in high dimensional settings. 
%
%Latent variable models are typically used with a large number of latent 
%variables. In this setting, and under appropriate conditions, the required 
%expectations for inference could be well approximated by Gaussian 
%expectations. Thus, we believe that our approach is applicable even in the 
%high-dimensional non-Gaussian or discrete setting: we can apply the 
%gradient estimators derived in section \ref{sec:learning} as an 
%approximation 
%in high-dimensional latent variable models and potentially obtain new 
%learning rules for these models.
%
%An additional feature of our approach is that it can easily be combined with 
%convolutional architectures and computation using GPUs to allow for scaling 
%to the high-dimensional settings we are now routinely faced with. More 
%investigation is required to fully explore the impact of the structure of the 
%recognition model and to allow more accurate covariance estimation. 
%This is particularly important in the high-dimensional setting where we lack 
%intuition regarding the characteristics of the posterior distribution. This and 
%other extensions form the basis of much future work.
We have introduced a general-purpose inference method for 
models with continuous latent variables. 
Our approach introduces a recognition model, which can be seen as a stochastic encoding of the data, to allow for efficient and tractable inference. 
We derived a lower bound on the marginal likelihood for the generative model and specified the structure and regularisation of the recognition model by exploiting recent advances in deep learning. 
By developing modified rules for backpropagation through stochastic 
layers, we derived an efficient inference algorithm that allows for joint 
optimisation of all parameters.
%We show competitive results on several datasets.
%Demonstratings
We show on several real-world data sets that the
model generates realistic samples, provides accurate imputations of 
missing data and can be a useful tool for high-dimensional data visualisation. 

==> 2014_icml_NGBR 2/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
There is an immense effort in machine learning and statistics to develop 
accurate and scalable probabilistic models of data. Such models are called 
upon whenever we are faced with tasks requiring probabilistic reasoning, 
such as prediction, missing data imputation and uncertainty estimation; or 
in simulation-based analyses, common in many scientific fields such as genetics, 
robotics and control that require generating a large number of 
independent samples from the model.

Recent efforts to develop generative models have focused on directed models, 
since samples are easily obtained by ancestral sampling from the generative 
process. Directed models such as belief networks and similar latent variable 
models \citep{dayan1995, frey1996, saul1996mean, book:bartholomew, 
uria2013, gregor2013} can be easily sampled from, but in most cases, efficient 
inference algorithms have remained elusive.
These efforts, combined with the demand for accurate probabilistic inferences 
and fast simulation, lead us to seek generative models that are
i) \textit{deep}, since hierarchical architectures allow us to capture complex 
structure in the data,
ii)  allow for \textit{fast sampling} of fantasy data from the inferred model, and
iii) are computationally \textit{tractable and scalable} to high-dimensional 
data. 

We meet these desiderata by introducing a class of deep, directed generative models with Gaussian latent variables at each layer. To allow for efficient and tractable inference, we 
use introduce an approximate representation of the posterior over the latent variables using a recognition model that acts as a stochastic encoder of the data.
%introduce a recognition model that represents an approximate posterior distribution over the latent variables, and that can be interpreted as a stochastic encoder of the data. 
For the generative model, we derive the objective function for optimisation using variational principles; for the recognition model, we specify its structure and regularisation by exploiting recent advances in deep learning. 
Using this construction, we can train the entire model by a modified form of gradient 
backpropagation that allows for optimisation of the parameters of  both the 
generative and recognition models jointly. 
%This allows for an algorithm with 
%the same complexity as that of an auto-encoder or related mean-field 
%%%approaches. 

We build upon the large body of prior work (in section 
\ref{sec:relatedWork}) and make the following contributions:
\begin{itemize}
\vspace{-4mm}
\setlength{\itemsep}{1pt}\setlength{\parskip}{0pt} \setlength{\parsep}{0pt}
\item We combine ideas from deep neural networks and probabilistic latent 
variable modelling to derive a general class of deep, non-linear latent 
Gaussian models (section \ref{sec:model}).
\item We present a new approach for scalable variational inference that 
allows for joint optimisation of both variational and model parameters by 
exploiting the properties of latent Gaussian distributions and gradient 
backpropagation (sections \ref{sec:stochBP} and \ref{sec:learning}).
\item We provide a comprehensive and systematic evaluation of the model 
demonstrating its applicability to problems in simulation, visualisation, 
prediction and missing data imputation (section \ref{sec:Results}).
\end{itemize}

==> 2014_icml_NGBR 2/learning.tex <==
\vspace{-3mm}
\section{Scalable Inference in DLGMs}
\label{sec:learning}
%In this section we derive a scalable inference algorithm for DLGMs. 
We use the matrix $\vV$ to refer to the full data set of size 
$N\times D$ with observations $\vv_n = [v_{n1}, \ldots, v_{nD}]^\top$. 

\vspace{-2mm}
\subsection{Free Energy Objective}
To perform inference in DLGMs we must integrate out the effect of 
any latent variables -- this requires us to compute the integrated or marginal 
likelihood. 
In general, this will be an intractable integration and instead we optimise a 
lower bound on the marginal likelihood. We introduce an 
approximate posterior distribution $q(\cdot)$ and apply Jensen's inequality 
following the variational principle \citep{beal2003} to obtain:
\vspace{-3mm}
\begin{align}
\mathcal{L}(\vV) &= -\log p(\vV) = -\log \int p(\vV |\vxi,\vtheta^g) 
p(\vxi,\vtheta^g)  d\vxi \nonumber \\
& = -\log \int  \frac{ q(\vxi)}{q(\vxi) } p(\vV |\vxi,\vtheta^g) 
p(\vxi,\vtheta^g)
 d\vxi  \label{eq:FE} \\ 
{\leq} \FE(\vV) & \!=\!D_{KL}[q(\vxi) \| p(\vxi)]\! -\! \expect{q}{\log p(\vV 
|\vxi,\!\vtheta^g)p(\vtheta^g)} .\nonumber
\end{align}
This objective consists of two terms: the first 
is the KL-divergence between the variational distribution and the prior 
distribution (which acts a regulariser), and the second is a reconstruction 
error. 

We specify the approximate posterior as  a distribution $q(\vxi | \vv)$ that is \textit{conditioned} on the observed data. This distribution can be specified as any directed acyclic graph where each node of the graph is a Gaussian conditioned, through linear or non-linear transformations, on its parents. The joint distribution in this case is non-Gaussian, but stochastic backpropagation can still be applied.  

For simplicity, we use a $q(\vxi | \vv)$ that is a Gaussian distribution that factorises across 
the $L$ layers (but not necessarily within a layer):
\vspace{-2mm}
\begin{equation}
q(\vxi | \vV, \vtheta^r) = \prod_{n=1}^N \prod_{l=1}^L  \N\left( 
\vxi_{n,l} | 
\vmu_{l}(\vis_n), \vC_l(\vis_n)  \right),
\label{eq:Q}
\end{equation}
where the mean $\vmu_l(\cdot)$ and covariance $\vC_l(\cdot)$ are generic maps represented by 
deep neural networks. Parameters of the $q$-distribution are denoted by the vector $\vtheta^r$.

For a Gaussian prior and a Gaussian recognition model, the KL term in \eqref{eq:FE} can be computed analytically and the free energy becomes:
\vspace{-1mm}
\begin{align}
D_{\!KL}&[\N(\vmu,\!\vC)\| \N(\vzero, \!\vI)] \!=\! \tfrac{1}{2}\! 
\left[\textrm{Tr}(\!\vC\!)\!-\!\log|\vC| \!+\! \vmu\!^\top\!\!\vmu \!-\!D \right], 
\nonumber \\
\FE(\vV) &= -\sum_n
\E_{q} \left[ \log p(\vis_n| \hid(\vxi_n) ) \right]  
 + \tfrac{1}{2 \kappa} \Vert \vtheta^g\Vert ^2 \nonumber \\
&+\! \frac{1}{2}\! \sum_{n,l}\! \left[ \Vert \vmu_{n,l} \Vert ^2 \!+ \!
\Tr(\vC _{n,l}) \! -\! \log \vert \vC_{n,l} \vert \!-\!1 \right]\!,\! 
\label{eq:FEsimp}
\end{align}
where $\Tr(\vC)$ and $\vert \vC \vert$ indicate the trace and the 
determinant of the covariance matrix $\vC$, respectively.

The specification of an approximate posterior distribution that is conditioned on the observed data is the first component of an efficient variational inference algorithm. We shall refer to the distribution $q(\vxi| \vv)$ \eqref{eq:Q} as a \textit{recognition model}, whose design is independent of the generative model. A recognition model allows us introduce a form of amortised inference \citep{gershman2014} for variational methods in which we share statistical strength by allowing for generalisation across the posterior estimates for all latent variables using a model. The implication of this generalisation ability is: faster convergence during training; and faster inference at test time since we only require a single pass through the recognition model, rather than needing to perform any iterative computations (such as in a generalised E-step). 

To allow for the best possible inference, the specification of the recognition model must be flexible enough to provide an accurate approximation of the posterior distribution -- motivating the use of deep neural networks. 
We regularise the recognition model by introducing additional noise, specifically, bit-flip or drop-out noise at the input layer and small additional Gaussian noise to samples from the recognition model. 
We use rectified linear activation functions as non-linearities for any deterministic layers of the neural network. We found that such regularisation is essential and without it the recognition model is unable to provide accurate inferences for unseen data points. 

%Using a recognition model shows that a number of perspectives can be viewed as variational inference in hierarchical non-linear latent Gaussian models: a) In deep learning, denoising auto-encoders have a direct correspondence with the recognition model as the encoder, which we describe in section \ref{sec:discussion}; b) In information theory, we obtain the minimum description length compression, where the recognition model is the compressor or coding distribution; c) In manifold learning, the recognition model is the operation that produces a low-dimensional embedding of the data, allowing for learning of projections better suited for Gaussian posteriors.
%
\vspace{-2mm}
\subsection{Gradients of the Free Energy}
To optimise \eqref{eq:FEsimp}, we use Monte Carlo methods for any expectations and use stochastic 
gradient descent for optimisation. For optimisation, we  require efficient estimators of the gradients 
of all 
terms in equation \eqref{eq:FEsimp} with respect to the parameters $\vtheta^g$ and $\vtheta^r$
of the generative  and the recognition models, respectively.

The gradients with respect to the $j$th generative parameter $\theta_j^g$  can 
be computed using:
\vspace{-2mm}
\begin{align}
\nabla_{ \theta_j^g } \FE (\vV)  &= -  \E_{q} \left[ \nabla_{\theta_j^g} \log 
p(\vV| \hid ) 
\right] +\tfrac{1}{\kappa}  \theta_j^g. \label{eq:dFEdThetaG}
\end{align}
An unbiased estimator of $\nabla_{ \theta_j^g } \FE (\vV)$ is obtained by 
approximating equation \eqref{eq:dFEdThetaG} with a small number of samples 
(or 
even a single sample)
from the recognition model $q$.

To obtain gradients with respect to the recognition parameters $\vtheta^r$, 
we use the rules for Gaussian backpropagation developed in section 
\ref{sec:stochBP}. To address the complexity of the Hessian in the general 
rule 
\eqref{eq:GBP}, we use the co-ordinate transformation for the Gaussian to 
write the gradient with respect to the factor matrix $\vR$ instead of the 
covariance $\vC$ (recalling $\vC = \vR \vR^\top$) derived in equation 
\eqref{eq:gradR}, where derivatives are computed for the function $f(\vxi) = \log p(\vis| \hid(\vxi))$.

The gradients of $\FE(\vis)$ in equation \eqref{eq:FEsimp} with 
respect to the variational mean $\vmu_l (\vis)$ and the factors 
$\vR_l(\vis)$ 
are:
\vspace{-2mm}
\begin{align}
\nabla_{\mu_l} \FE(\vis) 
&= -  \E_{q} \left[ \nabla_{\vxi_l} \log p(\vis| \hid(\xi) ) 
\right] + \vmu_l, \label{eq:dFEdMu} \\
\nabla_{R_{l,i,j}} \FE(\vis)
&= - \tfrac{1}{2}\E_{q} \left[ \epsilon_{l,j}
\nabla_{\xi_{l,i}} \log p(\vis| \hid(\vxi) ) 
\right] \nonumber\\
&+ \tfrac{1}{2}\nabla_{R_{l,i,j}}  \left[ \Tr \vC _{n,l}  - \log \vert \vC_{n,l} 
\vert \right], \label{eq:dFEdR}
\end{align}
where the gradients $\nabla_{R_{l,i,j}}  \left[ \Tr \vC _{n,l}  - \log \vert 
\vC_{n,l} 
\vert \right]$ are computed by backpropagation.
Unbiased estimators of the gradients \eqref{eq:dFEdMu} and 
\eqref{eq:dFEdR} are obtained jointly by 
sampling from the recognition model $\vxi \sim q(\vxi | \vis)$ (bottom-up 
pass) and updating the values of the generative model layers using 
equation \eqref{eq:HiddenGen} (top-down 
pass). 

Finally the gradients $\nabla_{ \theta_j^r } \FE (\vis)$ obtained from 
equations \eqref{eq:dFEdMu} and \eqref{eq:dFEdR} are:
\vspace{-2mm}
\begin{align}
\!\!\!\nabla_{\small{\vtheta^r}} \FE (\vis) \!=\! 
\! \nabla_{\small{\vmu}} \FE (\vis)\!^\top\! \frac{\partial \vmu}{\partial 
\vtheta^r}\! +\! \! \Tr \left(\!\nabla_{\small{\vR}} \FE(\vis)\frac{\partial 
\vR}{\partial 
\vtheta^r} \!\right) \!. \label{eq:dFEdThetaR}
\end{align}
The gradients \eqref{eq:dFEdThetaG} -- 
\eqref{eq:dFEdThetaR} are now used to descend the free-energy surface with respect to  
both the 
generative and recognition parameters in a single optimisation step. 
Figure \ref{fig:introCompGraph} shows the flow of computation in 
DLGMs. Our algorithm proceeds by first performing a forward pass (black 
arrows), consisting of a bottom-up (recognition) phase and a top-down 
(generation) phase, which updates the hidden activations of the recognition 
model and parameters of any Gaussian distributions, and then a backward 
pass 
(red arrows) in which gradients are computed using the appropriate 
backpropagation rule for deterministic and stochastic layers.
We take a descent step using:
\vspace{-1mm}
\begin{equation} 
\Delta \theta^{g,r} = -\Gamma^{g,r} {\nabla_{\theta^{g,r} } 
\FE(\vV)}, \label{eq:SGD}
\vspace{-1mm}
\end{equation}
where $\Gamma^{g,r}$ is a diagonal pre-conditioning matrix computed using the RMSprop 
heuristic\footnote{Described by G. Hinton, 
	`RMSprop: Divide the gradient by a running average of its recent 
		magnitude', in \textit{Neural networks for machine learning}, 
	Coursera lecture 6e, 2012.}. The learning 
procedure is summarised in algorithm 
\ref{alg:train}.
\vspace{1.5mm}
\begin{algorithm}[tbp]
  \caption{Learning in {\model}\!s}
  \label{alg:train}
\begin{algorithmic}
\WHILE{ hasNotConverged() }
\STATE $\vV \gets \text{getMiniBatch}()$
\STATE $\vxi_n \sim q(\xi_n | \vis_n)$ (bottom-up pass) eq. \eqref{eq:Q}
\STATE $\hid \leftarrow \hid(\xi)$ (top-down pass) eq. \eqref{eq:HiddenGen}
\STATE updateGradients() eqs \eqref{eq:dFEdThetaG} -- %\eqref{eq:dFEdMu}, 
%\eqref{eq:dFEdR}
\eqref{eq:dFEdThetaR}
\STATE $\vtheta^{g,r} \gets \vtheta^{g,r} + \Delta \vtheta^{g,r}$
\ENDWHILE
\end{algorithmic}
\end{algorithm}

\vspace{-3mm}
\subsection{Gaussian Covariance Parameterisation}
%\subsection{Designing the Recognition Model}
\label{sec:learning_covParam}

There are a number of approaches for parameterising the covariance matrix 
of the recognition model $q(\vxi)$. Maintaining a full covariance matrix 
$\vC$ in 
equation 
\eqref{eq:FEsimp} would 
entail an algorithmic complexity of $O(K^3)$ for training and sampling per layer, 
where $K$ is the number of latent variables per layer.

The simplest approach is to use a diagonal covariance matrix $\vC = 
\textrm{diag}(\vd)$, where $\vd$ is a $K$-dimensional vector. This 
approach is appealing since it allows for linear-time computation and 
sampling, but only allows for axis-aligned posterior distributions.

We can improve upon the diagonal approximation by 
parameterising the covarinace as a rank-1 matrix with a diagonal correction. 
Using a vectors $\vu$ and $\vd$, with $\vD = \textrm{diag}(\vd)$, we parameterise the precision 
 $\vC^{-1}$ as:
\vspace{-2mm}
\begin{equation}
\vC^{-1} = \vD + \vu \vu^\top. \label{eq:Cinv}
\vspace{-2mm}
\end{equation}
This representation allows for arbitrary rotations of the Gaussian distribution 
along one principal direction with relatively few additional parameters 
\citep{magdon-ismail2010a}. By application of the matrix inversion lemma (Woodbury identity), we obtain 
the covariance matrix in terms of $\vd$ and $\vu$ as:
\vspace{-2mm}
\begin{align}
& \vC  = \vD^{-1} + \eta \vD^{-1} \vu \vu^\top \vD^{-1}, \label{eq:C}  & 
\quad \eta = \tfrac{1}{\vu^\top \vD^{-1} \vu + 1}, \nonumber \\
& \log \vert \vC \vert  = \log \eta - \log \vert \vD \vert. 
\vspace{-2mm}
\end{align}
This allows both the trace $\Tr(\vC)$  and $\log \vert \vC \vert$ needed 
in the computation of the Gaussian KL, as well as their gradients, to be computed in $O(K)$ time per layer.

The factorisation $\vC = \vR \vR^\top$, with $\vR$ a matrix of the same size as 
$\vC$ and can be computed directly in terms of $\vd$ and $\vu$. One solution for $\vR$ is:
\begin{align}
\vR = \vD^{ -\frac{1}{2} } - \left[ \frac{1 - \sqrt{\eta}}{\vu^\top \vD^{-1} 
\vu} \right] \vD^{-1} \vu \vu^\top \vD^{ -\frac{1}{2} }.
\label{eq:R}
\end{align}
The product of $\vR$ with an arbitrary vector can be 
computed in $O(K)$ without computing $\vR$ explicitly. This also
allows 
us to sample efficiently from this Gaussian, since any Gaussian 
random variable $\vxi$ with mean $\vmu$ and covariance matrix $\vC = 
\vR \vR^\top$ can be written as
$\vxi = \vmu + \vR \vepsilon, \label{eq:XiR}$
where $\vepsilon$ is a standard Gaussian variate. 

Since this covariance parametrisation has linear cost in the number of latent 
variables, we can also use it to 
parameterise the variational distribution of all layers jointly, instead of the 
factorised assumption in \eqref{eq:Q}. 
%This could lead to more accurate posterior approximations. 

\subsection{Algorithm Complexity}
\label{sec:learning_algo}

The computational complexity of producing a sample from the 
generative model is $O(L\bar{K}^2)$,  where 
$\bar{K}$ is the average number of latent variables per layer and $L$ is the 
number of layers (counting both deterministic and stochastic layers). The computational 
complexity per training sample during training is also $O(L\bar{K}^2)$ --  the same as that of matching  auto-encoder.

==> 2014_icml_NGBR 2/macros.tex <==

\usepackage{amsmath, amsthm}
\usepackage{amsfonts}
\usepackage{amssymb}

% Generic math notations
\newcommand{\assign}{:=}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\eqsp}{\,}	% equal space between equations and punctuation
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\proc}[1]{\textsc{#1}}
\newcommand{\categorical}{\text{Cat}}

\newcommand{\E}{\mathbb{E}} %expectation
\newcommand{\FE}{\mathcal{F}} %free energy
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\Tr}{Tr} %matrix trace
\DeclareMathOperator{\diag}{diag} %matrix trace
\let\oldthebibliography=\thebibliography
  \let\endoldthebibliography=\endthebibliography
  \renewenvironment{thebibliography}[1]{%
    \begin{oldthebibliography}{#1}%
      \setlength{\parskip}{0.7ex}%
      \setlength{\itemsep}{0ex}%
}{\end{oldthebibliography}}
  
% Model specific
\newcommand{\model}{DLGM\hspace{1mm}} %model name
\newcommand{\hid}{\ensuremath{\mathbf{h}}} % hidden units
\newcommand{\vis}{\ensuremath{\mathbf{v}}} % Visible units
% Recognition model
\newcommand{\N}{\mathcal{N}} % Gaussian


%\usepackage[usenames]{color}
\definecolor{darkblue}{rgb}{0,0.05,0.35}
\definecolor{darkgreen}{rgb}{0,0.6,0}
\renewcommand{\comment}[1]{\textcolor{red}{[#1]}}
\newcommand{\scom}[1]{\textcolor{darkgreen}{[#1]}}
\newcommand{\dcom}[1]{\textcolor{blue}{[#1]}}

% Prob expressions
\newcommand{\Expon}[1]{\mathrm{Expon}\left( #1 \right )}
\newcommand{\Conj}[1]{\mathrm{Conj}\left(#1 s\right)}
\newcommand{\expect}[2]{\mathbb{E}_{#1}\left[#2\right]}

% vector symbols
\newcommand{\myvec}[1]{\mbox{$\mathbf{#1}$}}
\newcommand{\myvecsym}[1]{\mbox{$\boldsymbol{#1}$}}

\newcommand{\vzero}{\mbox{$\myvecsym{0}$}}
\newcommand{\vone}{\mbox{$\myvecsym{1}$}}

\newcommand{\valpha}{\mbox{$\myvecsym{\alpha}$}}
\newcommand{\vbeta}{\mbox{$\myvecsym{\beta}$}}
\newcommand{\vchi}{\mbox{$\myvecsym{\chi}$}}
\newcommand{\vdelta}{\mbox{$\myvecsym{\delta}$}}
\newcommand{\vDelta}{\mbox{$\myvecsym{\Delta}$}}
\newcommand{\vepsilon}{\mbox{$\myvecsym{\epsilon}$}}
\newcommand{\veta}{\mbox{$\myvecsym{\eta}$}}
\newcommand{\vgamma}{\mbox{$\myvecsym{\gamma}$}}
\newcommand{\vmu}{\mbox{$\myvecsym{\mu}$}}
\newcommand{\vlambda}{\mbox{$\myvecsym{\lambda}$}}
\newcommand{\vLambda}{\mbox{$\myvecsym{\Lambda}$}}
\newcommand{\vLambdaBar}{\mbox{$\overline{\vLambda}$}}
\newcommand{\vphi}{\mbox{$\myvecsym{\phi}$}}
\newcommand{\vPhi}{\mbox{$\myvecsym{\Phi}$}}
\newcommand{\vpi}{\mbox{$\myvecsym{\pi}$}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\mbox{$\myvecsym{\Psi}$}}
\newcommand{\vtheta}{\mbox{$\myvecsym{\theta}$}}
\newcommand{\vTheta}{\mbox{$\myvecsym{\Theta}$}}
\newcommand{\vsigma}{\mbox{$\myvecsym{\sigma}$}}
\newcommand{\vSigma}{\mbox{$\myvecsym{\Sigma}$}}
\newcommand{\vOmega}{\mbox{$\myvecsym{\Omega}$}}
\newcommand{\vtau}{\mbox{$\myvecsym{\tau}$}}
\newcommand{\vxi}{\mbox{$\myvecsym{\xi}$}}

\newcommand{\va}{\mbox{$\myvec{a}$}}
\newcommand{\vb}{\mbox{$\myvec{b}$}}
\newcommand{\vc}{\mbox{$\myvec{c}$}}
\newcommand{\vd}{\mbox{$\myvec{d}$}}
\newcommand{\ve}{\mbox{$\myvec{e}$}}
\newcommand{\vf}{\mbox{$\myvec{f}$}}
\newcommand{\vg}{\mbox{$\myvec{g}$}}
\newcommand{\vh}{\mbox{$\myvec{h}$}}
\newcommand{\vj}{\mbox{$\myvec{j}$}}
\newcommand{\vk}{\mbox{$\myvec{k}$}}
\newcommand{\vm}{\mbox{$\myvec{m}$}}
\newcommand{\vn}{\mbox{$\myvec{n}$}}
\newcommand{\vp}{\mbox{$\myvec{p}$}}
\newcommand{\vq}{\mbox{$\myvec{q}$}}
\newcommand{\vr}{\mbox{$\myvec{r}$}}
\newcommand{\vs}{\mbox{$\myvec{s}$}}
\newcommand{\vt}{\mbox{$\myvec{t}$}}
\newcommand{\vu}{\mbox{$\myvec{u}$}}
\newcommand{\vv}{\mbox{$\myvec{v}$}}
\newcommand{\vw}{\mbox{$\myvec{w}$}}
\newcommand{\vws}{\mbox{$\vw_s$}}
\newcommand{\vwh}{\mbox{$\hat{\vw}$}}
\newcommand{\vx}{\mbox{$\myvec{x}$}}
\newcommand{\vxt}{\mbox{$\myvec{\tilde{x}}$}}
\newcommand{\vy}{\mbox{$\myvec{y}$}}
\newcommand{\vyt}{\mbox{$\myvec{\tilde{y}}$}}
\newcommand{\vz}{\mbox{$\myvec{z}$}}

\newcommand{\vA}{\mbox{$\myvec{A}$}}
\newcommand{\vB}{\mbox{$\myvec{B}$}}
\newcommand{\vC}{\mbox{$\myvec{C}$}}
\newcommand{\vD}{\mbox{$\myvec{D}$}}
\newcommand{\vE}{\mbox{$\myvec{E}$}}
\newcommand{\vF}{\mbox{$\myvec{F}$}}
\newcommand{\vG}{\mbox{$\myvec{G}$}}
\newcommand{\vH}{\mbox{$\myvec{H}$}}
\newcommand{\vI}{\mbox{$\myvec{I}$}}
\newcommand{\vJ}{\mbox{$\myvec{J}$}}
\newcommand{\vK}{\mbox{$\myvec{K}$}}
\newcommand{\vL}{\mbox{$\myvec{L}$}}
\newcommand{\vM}{\mbox{$\myvec{M}$}}
\newcommand{\vN}{\mbox{$\myvec{N}$}}
\newcommand{\vO}{\mbox{$\myvec{O}$}}
\newcommand{\vP}{\mbox{$\myvec{P}$}}
\newcommand{\vQ}{\mbox{$\myvec{Q}$}}
\newcommand{\vR}{\mbox{$\myvec{R}$}}
\newcommand{\vS}{\mbox{$\myvec{S}$}}
\newcommand{\vT}{\mbox{$\myvec{T}$}}
\newcommand{\vU}{\mbox{$\myvec{U}$}}
\newcommand{\vV}{\mbox{$\myvec{V}$}}
\newcommand{\vW}{\mbox{$\myvec{W}$}}
\newcommand{\vX}{\mbox{$\myvec{X}$}}
%\newcommand{\vXs}{\mbox{$\vX_{\vs}$}}
\newcommand{\vXs}{\mbox{$\vX_{s}$}}
\newcommand{\vXt}{\mbox{$\myvec{\tilde{X}}$}}
\newcommand{\vY}{\mbox{$\myvec{Y}$}}
\newcommand{\vZ}{\mbox{$\myvec{Z}$}}


%Latex theorem/proposition/lemma environments
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}




==> 2014_icml_NGBR 2/model.tex <==
\vspace{-3mm}
\section{Deep Latent Gaussian Models}
\label{sec:model}
Deep latent Gaussian models (DLGMs) are a general class of deep directed graphical models that consist of Gaussian latent variables at each layer of a processing hierarchy.
The model consists of $L$ layers of latent variables. To generate a sample from the model, we begin at the top-most layer ($L$) by drawing from a Gaussian distribution. 
The activation $\vh_{l}$ at any lower layer is formed by a non-linear 
transformation of the layer above $\vh_{l+1}$, perturbed by Gaussian 
noise. 
We descend through the hierarchy and generate observations $\vv$ by 
sampling from the observation likelihood using the activation of the lowest layer 
$\vh_1$. This process is 
described graphically in figure \ref{fig:graphModel}.
\begin{figure}[tb]
	\centering
	\subfigure[]{
		%0.19
		\includegraphics[width=0.22\columnwidth]{introA.pdf}
		\label{fig:graphModel}}
	%\subfigure[]{\raisebox{4mm}{
	%0.2
	%\includegraphics[width=0.2\columnwidth]{introB.pdf}}
	%\label{fig:equivGraph} 
	%}
	\subfigure[]{
		%0.49
		\includegraphics[width=0.7\columnwidth]{introC.pdf} 
		\label{fig:introCompGraph}}
	\vskip -0.08in 
	\caption{(a) Graphical model for DLGMs 
		\eqref{eq:LogLikeStandard}. 
		%(b) Graphical model corresponding to equation 
		%\eqref{eq:LogLike}.
		(b) The corresponding computational graph. 
		Black arrows indicate the forward pass of 
		sampling 
		from the recognition and generative models: Solid lines indicate propagation of deterministic activations,  dotted lines 
		indicate propagation of samples. 
		Red arrows indicate the 
		backward pass for gradient computation: Solid lines indicate paths where deterministic backpropagation is used, 
		dashed arrows indicate stochastic backpropagation.}
	\label{figure:introModel}
	\vspace{-5mm}
\end{figure} 

This generative process is described as follows:
\vspace{-2mm}
\begin{align}
\vxi_l & \sim \N(\vxi_l | \vzero, \vI), \quad l = 1, \ldots, L \\
\hid_{L} &= \vG_{L} \vxi_{L}, \label{eq:xL} \\
\hid_{l} &= T_l(\hid_{l+1}) + \vG_{l} \vxi_{l}, \quad l =1 \ldots L-1 
\label{eq:HiddenGen} \\
\vis & \sim  \pi(\vis | T_0(\hid_{1})),
\label{eq:Visible}
\end{align}
where $\vxi_l$ are mutually independent Gaussian variables. The 
transformations $T_l$ represent multi-layer perceptrons (MLPs) and 
$\vG_l$ are matrices. At the visible layer, the data is generated from any 
appropriate distribution $\pi(\vis | 
\cdot)$ whose parameters are specified by a transformation of the first 
latent layer. 
Throughout the paper we refer 
to the set of parameters in  this generative model  by $\vtheta^g$, i.e. the parameters of the maps $T_l$ and the matrices $G_l$. This 
construction allows us to make use of as many deterministic and stochastic 
layers as needed.
We adopt a 
weak Gaussian prior over $\vtheta^g$, $p(\vtheta^g) = \N(\vtheta| \vzero, 
\kappa\vI)$.

The joint probability distribution of this model can be expressed in two equivalent ways:
\begin{align}
& p(\vis,\! \hid)\! =\! p(\!\vis| \hid_1, \!\vtheta^g ) p(\hid_L | \vtheta^g) 
p(\!\vtheta^g\!)
\!\!\prod_{l=1}^{L 
- 1}\!\! p_l( \hid_l | \hid_{l\!+\!1}, \!\vtheta^g )\label{eq:LogLikeStandard} 
\\
& p(\vis,\!\vxi)\! = p(\vis| \hid_1( \vxi_{1 \ldots L} ), \vtheta^g ) 
p(\vtheta^g) 
\prod_{l=1}^{L} 
 \N(\vxi| \vzero, \vI). \label{eq:LogLike}
\end{align}
The conditional distributions $p( \hid_l | \hid_{l+1} )$ are implicitly 
defined by equation \eqref{eq:HiddenGen} and are Gaussian distributions 
with mean $\vmu_l = T_l(\hid_{l+1})$ and covariance $\vS_l = \vG_l 
\vG_l^\top$. Equation \eqref{eq:LogLike} makes explicit that this 
generative model works by applying a complex non-linear transformation to 
a spherical Gaussian distribution $p(\vxi) = \prod_{l=1}^{L} 
\N(\vxi_l| \vzero, \vI)$ such that the transformed 
distribution tries to match the empirical distribution. A graphical model 
corresponding to equation \eqref{eq:LogLikeStandard} is shown in figure
\ref{figure:introModel}(a). 
%We discuss this 
%in more detail in appendix \ref{app:altView}. 

This specification for deep latent Gaussian models (DLGMs) generalises a number 
of well known models. 
When we have only one layer of latent variables and use a linear 
mapping $T(\cdot)$, we recover \textit{factor analysis} \citep{book:bartholomew} -- more general 
mappings allow for a non-linear factor analysis \citep{lappalainen2000bayesian}. When the mappings 
are of the form $T_l(\hid) = \vA_l f(\hid) + \vb_l$, for simple element-wise 
non-linearities $f$ such as the probit function or the rectified linearity, we 
recover the \textit{non-linear Gaussian belief network} \citep{frey1999a}. We describe the relationship to other existing models in 
section \ref{sec:relatedWork}. Given this specification, our key task is to 
develop a method for tractable inference. A number of 
approaches are known and widely used, and include: mean-field variational EM \citep{beal2003}; the wake-sleep algorithm 
\citep{dayan2000}; and stochastic variational methods and related control-variate 
estimators \citep{wilson1984variance, Williams1992, hoffman2012stochastic}. We 
also follow a stochastic variational approach, but shall develop an alternative to 
these existing 
inference algorithms that overcomes many of their limitations and that is both scalable and efficient.


==> 2014_icml_NGBR 2/relatedWork.tex <==
%\vspace{-2mm}
\section{Discussion}
\label{sec:discussion}
\label{sec:relatedWork}
%\vspace{-2mm}
\textbf{Directed Graphical Models.} 
%There is a broad existing literature on related directed graphical models.
% and our  specification for deep latent Gaussian models  
%generalises a number of well known models. 
%As mentioned in section \ref{sec:model}, 
DLGMs form a unified family of models that includes factor analysis \citep{book:bartholomew}, non-linear factor analysis \citep{lappalainen2000bayesian}, and non-linear Gaussian belief networks \citep{frey1999a}.
Other related models include
sigmoid belief networks \citep{saul1996mean} and
%are closely related and are models with Bernoulli variables at every layer. 
%Both these models are trained by a mean-field variational EM algorithm. 
deep 
auto-regressive networks \citep{gregor2013}, which use 
auto-regressive 
Bernoulli distributions at each 
layer instead of Gaussian distributions. The Gaussian process latent 
variable model and deep Gaussian processes
\citep{lawrence2005probabilistic, damianou2013} form the non-parametric analogue of 
our model and employ Gaussian process priors over the non-linear functions 
between each layer. 
The neural auto-regressive density estimator (NADE) \citep{larochelle2011, uria2013} 
uses function approximation to model conditional distributions within a 
directed acyclic graph. 
NADE is amongst the most competitive generative models currently available, 
but has several limitations,
such as the inability to allow for deep representations and difficulties in 
extending to locally-connected models (e.g., through the use of 
convolutional layers),  preventing it from scaling easily to 
high-dimensional data.

\textbf{Alternative latent Gaussian inference.} Few of the alternative approaches for inferring latent Gaussian distributions meet the desiderata for scalable inference we seek. 
The Laplace approximation has been concluded to be a poor approximation in general, in addition to being computationally expensive.
INLA is restricted to models with few hyperparameters ($<10$), whereas our interest is in 100s-1000s.
EP cannot be applied to latent variable models due to the inability to match moments of the joint distribution of latent variables and model parameters. % (hybrid EP-VB is used as a solution). 
Furthermore, no reliable methods exist for moment-matching with means and covariances formed by non-linear transformations -- linearisation and importance sampling are two, but are either inaccurate or very slow. Thus, the the variational approach we present remains a general-purpose and competitive approach for inference.

\textbf{Monte Carlo  variance reduction.} 
%\label{sec:learning_varAnalysis}
%When Monte Carlo methods are used to evaluate expectations, great care 
%must be taken to ensure efficient estimation by reducing the variance of the 
%simulation estimates. 
\textit{Control variate} methods are amongst the most 
general and 
effective techniques for variance reduction when Monte Carlo methods are used \citep{wilson1984variance}. One 
popular approach is the
%Other approaches for gradient estimation are typically used in the literature. 
%The most general approaches are policy-gradient methods such as 
REINFORCE algorithm \citep{Williams1992}, since it is simple to implement 
and applicable to both discrete and continuous  
models, though control variate methods are becoming increasingly popular 
for variational inference problems \citep{hoffman2012stochastic, 
	blei2012variational, ranganath2013, salimans2014}. Unfortunately, such 
estimators  have the undesirable property 
that their variance scales linearly with the number of independent random 
variables in the target function, while the variance of GBP is bounded by a 
constant: for $K$-dimensional latent variables the variance of 
REINFORCE scales as $O(K)$, whereas GBP scales as $O(1)$ (see appendix \ref{ap:var_reinforce}).

An important family of alternative estimators is based on \textit{quadrature and series 
	expansion methods} \citep{HonkelaV04, lappalainen2000bayesian}. These methods
have low-variance at the price of introducing biases in the estimation. More 
recently a combination of the series expansion and control variate 
approaches has been proposed by \citet{blei2012variational}.

A very general alternative 
is the \textit{wake-sleep algorithm} 
\citep{dayan1995}.  The wake-sleep algorithm can perform well, but it fails to optimise a single consistent objective function and there is 
thus no guarantee that optimising it leads to a decrease in the free energy (\ref{eq:FE}). 
%But it has been shown to work well in some small practical examples.

\textbf{Relation to denoising auto-encoders.} 
Denoising auto-encoders (DAE) \citep{vincent2010} introduce a 
random corruption to the encoder network and attempt to minimize the 
expected  reconstruction error under this corruption noise with additional 
regularisation terms. In our variational approach, the 
recognition distribution $q(\vxi|\vis)$ can be interpreted as a stochastic 
encoder in the DAE setting. There is then a direct correspondence between the expression for the free energy 
(\ref{eq:FE}) and the reconstruction 
error and regularization terms used in denoising auto-encoders (c.f. 
equation (4) of \citet{bengio2013}). Thus, we can see denoising auto-encoders as a realisation of 
variational inference in latent variable models.

The key difference is that the 
form of encoding `corruption' and regularisation terms used in our model 
have been derived directly using the variational principle to provide a strict 
bound on the marginal likelihood of a known directed graphical model 
that allows for easy generation of samples. 
DAEs can also be used as generative models by simulating from a Markov chain \citep{bengio2013,bengio2013deep}.
But the behaviour of these Markov chains will be very problem specific, 
and we lack consistent tools to evaluate their convergence. 
%Our preference is then to favour an approach where these considerations do not enter 
%into the design and evaluation of the model. We instead use DLGMs as a variational auto-encoder 
%that maintains the correspondence to DAEs, but for which the generative model is always known.

%While denoising auto-encoders 
%are trained by backpropagation, our modified backpropagation rules 
%provides unbiased estimators that account for the gradients through 
%the mean as well as the covariance. 

%Using a recognition model shows that a number of perspectives can be seen as variational inference in hierarchical non-linear latent Gaussian models: a) In deep learning, denoising autoencoders have a direct correspondence as we described; b) In information theory, we obtain the minimum description length compression where the recognition model is the compressor or coding distribution. c) In manifold learning, the recognition model is the operation that produces a low dimensional embedding of the data, allowing for learning of projections better suited for Gaussian posteriors. 


%\textbf{Further scalability.} 
%Our model can be easily combined with locally 
%connected 
%architectures (e.g., convolutions) for scalability to very large image data sets.
%Furthermore, the model can be constructed  with a variety of continuous distributions other than the 
%Gaussian, such as non-negative or sparsity-promoting latent variables, widening the range of potential applications (see appendix
%\ref{app:otherStochBPrule}).


==> 2014_icml_NGBR 2/simulations.tex <==
\vspace{-3mm}
\section{Results}
\label{sec:Results}
Generative models have a number of applications in simulation, prediction, 
data visualisation, missing data imputation and other forms of probabilistic 
reasoning. We describe the testing methodology we use and present results 
on a number of these tasks. 
\vspace{-2mm}

\subsection{Analysing the Approximate Posterior}
\begin{figure*}[tbp]
	\centering
	\subfigure[Diagonal covariance]{
		\includegraphics[height = 2cm]{image6}
		\includegraphics[height = 2cm]{image7}
		\includegraphics[height = 2cm]{image8}}
	\hspace{0.25cm}
	\subfigure[Low-rank covariance]{
		\includegraphics[height = 2cm]{posteriorMap_3}
		\includegraphics[height = 2cm]{posteriorMap_2}
		\includegraphics[height = 2cm]{posteriorMap_32}}
	\hspace{0.25cm}
	\subfigure[Performance]{
		\includegraphics[height = 2cm]{barplot_mnist-crop}}
	%mnistBoxPlot-crop
	\vskip-0.14in
	\caption{(a, b) Analysis of the true  vs. approximate posterior for
		MNIST. 
		%The grey regions show the true posterior distribution, green 
		%markers indicate samples from the prior distribution, blue markers are 
		%samples from the recognition model, and the red marker indicates the MAP 
		%estimate. 
		Within each image we show four views of the same posterior, 
		zooming in on the region centred on the MAP (red) estimate. 
		%The top-left regions are 
		%centred at the latent's origin and span values from $-4$ to $4$ in both 
		% axes.
		(c) Comparison of test log likelihoods. %for different inference algorithms.
		}
	\label{figure:MNIST_POSTERIOR}
	\vspace{-3mm}
\end{figure*} 
%The specification of the recognition model affects how well we are able to 
%capture the statistics of the data and the accuracy and efficiency of the 
%learning.  

%We examine the quality of the approximate posterior distribution 
%learnt by the recognition model in comparison to the true posterior 
%distribution, and gain insight into the suitability of the latent Gaussian construction by training a DLGM using the binarised 
%MNIST data set 
%of handwritten images. The images are of size 28$\times$28 pixels, and we use 
%the binarised data set 
%from \citet{larochelle2011}.

We use sampling to evaluate the true posterior distribution for a number of 
MNIST digits using the binarised data set from \citet{larochelle2011}.
%under the diagonal and the structured covariance 
%parameterisation of the recognition model described in section 
%\ref{sec:learning_covParam}. 
We visualise the posterior distribution for a 
model with two Gaussian latent variables in figure 
\ref{figure:MNIST_POSTERIOR}. The true posterior distribution is shown by 
the grey regions and was computed by importance sampling with a large 
number of particles aligned in a grid between -5 and 5. In figure 
\ref{figure:MNIST_POSTERIOR}(a) we see that these posterior distributions  
are elliptical or spherical in shape and thus, it is reasonable to assume that 
they can be well approximated by a Gaussian. Samples from the 
prior (green) are spread widely over the space and very few 
samples fall in the region of significant posterior mass, explaining the 
inefficiency of estimation methods that rely on samples from the prior. 
Samples from the recognition model (blue) are concentrated on 
the posterior mass, indicating that the recognition model has learnt the 
correct posterior statistics, which should lead to efficient learning. 
\begin{table}[tbp]
\vspace{-3mm}
\centering
\scriptsize
\caption{Comparison of negative log-probabilities on the test set for the binarised MNIST data. }
\label{tab:mnist}
\begin{tabular}{lc}
\hline
\textbf{Model} & $-\ln p(\mathbf{v})$ \\
\hline \hline
Factor Analysis & $106.00$ \\
NLGBN \citep{frey1999a} & $95.80$ \\
Wake-Sleep \citep{dayan2000} & 91.3\\
DLGM diagonal covariance & $87.30$ \\
DLGM rank-one covariance & $86.60$ \\
\hline
\multicolumn{2}{c}{\tiny\textit{Results below from \citet{uria2013}}} \\
MoBernoullis K=10 & 168.95 \\
MoBernoullis K=500 & 137.64 \\
RBM (500 h, 25 CD steps) approx. & 86.34\\
DBN 2hl approx. & 84.55\\
NADE 1hl (fixed order) & 88.86\\
NADE 1hl (fixed order, RLU, minibatch) & 88.33\\
EoNADE 1hl (2 orderings) & 90.69 \\
EoNADE 1hl (128 orderings) & 87.71 \\
EoNADE 2hl (2 orderings) & 87.96 \\
EoNADE 2hl (128 orderings) & 85.10 \\
\hline
\end{tabular}
%\vskip -3ex
\vspace{-7mm}
\end{table}
\newline \newline In figure \ref{figure:MNIST_POSTERIOR}(a) we see that samples from the 
recognition model are aligned to the axis and do not capture the posterior 
correlation. The correlation is captured using the structured covariance model
in
figure \ref{figure:MNIST_POSTERIOR}(b).
Not all posteriors are Gaussian in shape, but the recognition places mass in 
the best location possible to provide a reasonable approximation. As a benchmark for comparison, the performance in terms of test log-likelihood 
%on the MNIST data is shown for four algorithms on the same model 
is shown in figure \ref{figure:MNIST_POSTERIOR}(c), using the same 
architecture, for factor 
analysis (FA), the wake-sleep algorithm, 
and our approach using both the diagonal and structured covariance approaches. For this experiment, the generative model consists of 100 latent variables feeding into a deterministic layer of 300 nodes, which then feeds to the observation likelihood. We use the same structure for the recognition model.
%architecture in figure \ref{figure:MNIST_POSTERIOR}(c). We compare factor 
%analysis (FA), the wake-sleep algorithm, 
%and our approach using both a diagonal and low-rank covariances. 
%\vspace{-2mm}
\subsection{Simulation and Prediction}
\begin{figure*}[tbp]
	\centering
	\subfigure[Left: Training 
	data. Middle: Sampled pixel probabilities. Right: Model samples]{
		\frame{
			\includegraphics[height=3.8cm]{dataSample_49}}
		%\hspace{1cm}
		\frame{
			\includegraphics[height=3.8cm]{modelSample_49}}
		%\hspace{1cm}
		\frame{
			\includegraphics[height=3.8cm]{modelSamplePixel_49}}
		\label{figure:MNIST}
	}
	\hspace{0.5cm}
	\subfigure[2D embedding.]{
		\includegraphics[height = 3.8cm]{posteriorMapColored_50}
		\label{fig:mnist_embedding}}
	\vspace{-4mm}
	\caption{Performance on the MNIST dataset. For the visualisation, each colour corresponds to one of the digit classes.}
	\vspace{-2mm}
\end{figure*} 
\begin{figure*}[tbp]
	\centering
	\subfigure[NORB]{
		\includegraphics[height = 2.6cm]{dataSamples_NORB_cropped}
		\includegraphics[height = 2.6cm]{modelSamples_NORB_cropped}
		\label{figure:NORB}
	}
	\subfigure[CIFAR]{
		\includegraphics[height = 2.6cm]{dataSamples_CIFAR10_8x8patches}
		\includegraphics[height = 2.6cm]{modelSamples_CIFAR10_8x8patches_2}
		\label{figure:CIFAR10}
	}
	\subfigure[Frey]{
		\includegraphics[height=2.6cm]{dataSamples_FreyFaces}
		\includegraphics[height=2.6cm]{modelSample_15}
		\label{fig:freyFaces}
	}
	\vspace{-3mm}
	\caption{Sampled generated from DLGMs for three data sets: (a) NORB, (b) CIFAR 10, (c) Frey faces. In all images, the left image shows samples from the 
		training data and the right side shows the generated samples.}
	\vspace{-3mm}
\end{figure*}
%\vspace{-2mm}
We evaluate the performance of a three layer latent Gaussian model on the 
MNIST data set. The model consists of two deterministic layers with 200 
hidden units and a stochastic layer of 200 latent variables. We use 
mini-batches of 200 observations and trained the model using stochastic backpropagation. 
Samples from this model are shown in figure \ref{figure:MNIST}. We also 
compare the test log-likelihood to a large number of existing approaches 
in table \ref{tab:mnist}. We used the binarised dataset as in 
\citet{uria2013} and quote the log-likelihoods in the lower part of the 
table from this work. These results show that our approach is competitive with 
some of the best models currently available. The generated digits also 
match the true data well and visually appear as good as some of the best 
visualisations from these competing approaches. 

We also analysed the performance of our model on three high-dimensional 
real image data sets. The NORB object recognition data set consists of 
$24,300$ images that are of size $96 \times 96$ pixels. We use a 
model consisting of 1 deterministic layer of 400 hidden units and 
one stochastic layer of 100 latent variables. Samples produced from this 
model are shown in figure \ref{figure:NORB}. The CIFAR10 natural images 
data set consists of $50,000$ RGB images that are of size $32 
\times 32$ pixels, which we split into random $8 \times 8$ patches. We use 
the same 
model as used for the MNIST experiment and show samples from the model 
in figure \ref{figure:CIFAR10}. The Frey faces data set consists of almost 
$2,000$ images of different facial expressions
%\footnote{Images of Brendan Frey. Data from \url{http://www.cs.nyu.edu/~roweis/data.html}} 
of size 
$28 \times 20$ pixels. 

\subsection{Data Visualisation}
Latent variable models are often 
used for visualisation of 
high-dimensional data sets. We project the MNIST data set to a 
2-dimensional latent space and use this 2D embedding as a visualisation 
of the data --  an embedding for MNIST is shown in 
figure \ref{fig:mnist_embedding}. The classes separate into different 
regions,  suggesting that such embeddings can be useful in understanding the structure of high-dimensional data sets.

\subsection{Missing Data Imputation and Denoising}
We demonstrate the ability of the model to impute missing data using the street view house numbers (SVHN) data set \citep{SVHNdata}, which consists of $73,257$ images of size $32 \times 32$ pixels, and the Frey faces and MNIST data sets. The performance of the model is shown in figure \ref{fig:mnist_completion}. 

We test the imputation ability under two different missingness types 
\citep{little1987statistical}: Missing-at-Random (MAR), where we consider 
60\% and 80\% of the pixels to be missing randomly, and Not 
Missing-at-Random (NMAR), where we consider a square region of the image 
to be missing.
The model produces very good completions in both test cases. There is uncertainty in the identity of the image and this is
reflected in the errors in these completions as the resampling procedure is 
run (see transitions from digit 9 to 7, and digit 8 to 6 in figure 
\ref{fig:mnist_completion} ). This further demonstrates the ability of the 
model to capture the diversity of the underlying data. 
We do not integrate over the missing values, 
but use a procedure that simulates a Markov chain that we show converges 
to the true marginal distribution of missing given observed pixels. The 
imputation procedure is discussed in appendix \ref{ap:ImageCompletion}.
\begin{figure}[tb]
\centering
\frame{\includegraphics[width = 8cm]{imageCompletion_rand60_12}}
\frame{\includegraphics[width = 8cm]{imageCompletion_rand60_39}}
\frame{\includegraphics[width = 8cm]{imageCompletion_rand60_40}}
\vskip 4px
\frame{\includegraphics[width = 8cm]{imageCompletion_rand50_15}}
\vskip 4px
\frame{\includegraphics[width = 8cm]{imageCompletion_rand60_50}}
\vskip 4px
\frame{\includegraphics[width = 8cm]{imageCompletion_rand80_50}}
\vskip 4px
\frame{\includegraphics[width = 8cm]{imageCompletion_center_50}}
\caption{Imputation results:  Row 1, SVHN. Row 2, Frey faces.
	Rows 3--5, MNIST. Col. 1 shows the true data. Col. 2 shows pixel locations set as missing in grey. The remaining columns show imputations for 15 iterations. 
	%Row 1: 60\% missingness. Row 2: 80\% missingness. Row 3: 5x5 patch missing. Row 4: 60\% missingness. Row 5: 50\% missingness.
	}
\label{fig:mnist_completion}
\vspace{-6mm}
\end{figure}







==> 2014_icml_NGBR 2/stochasticBP.tex <==
\vspace{-3mm}
\section{Stochastic Backpropagation}
\label{sec:stochBP}
Gradient descent methods in latent variable models typically require 
computations of the form $\nabla_\theta \expect{q_\theta}{f(\vxi)}$, where 
the expectation is taken with respect to a distribution $q_\theta(\cdot)$ with 
parameters
$\vtheta$, and $f$ is 
a loss function that we assume to be integrable and smooth. This quantity 
is difficult to compute directly since i)  the expectation is unknown for most problems, and ii) there is an indirect dependency on the parameters of $q$ over which the expectation is taken. 
%Furthermore, such expectations are computed by Monte Carlo methods, which 
%require special care in order to obtain low variance estimators. 

We now develop the key identities that are used to allow for efficient inference by exploiting specific properties of the problem of computing gradients through random variables. We refer to this computational strategy as \textit{stochastic backpropagation}.
\vspace{-2mm}
\subsection{Gaussian Backpropagation (GBP)}
When the distribution $q$ is a
$K$-dimensional Gaussian $\N(\vxi | \vmu, \vC)$  
the required gradients can be computed 
using the Gaussian gradient identities:
\vspace{-1mm}
\begin{align}
\nabla_{\mu_i} \E_{ \tiny{\N(\vmu,\vC)} } \left[ f(\vxi) \right ] &= \E_{ 
\tiny{\N(\vmu,\vC)} } \left[
\nabla_{\xi_i} f(\vxi) \right], \label{eq:bonnet} \\
\nabla_{C_{ij}} \E_{ \tiny{\N(\vmu,\vC) } }\left [ f(\vxi) \right ] &= \tfrac{1}{2}  \E_{ 
\tiny{\N(\vmu,\vC)} } \left [ 
\nabla^2_{\xi_i,\xi_j} f(\vxi) \right], \label{eq:price}
\end{align}
which are due to the theorems by \citet{bonnet1964} and  \citet{price1958}, 
respectively. These equations are true in expectation 
 for any integrable and smooth function $f(\vxi)$. Equation 
\eqref{eq:bonnet} is a direct consequence of the location-scale 
transformation for the Gaussian (discussed in section 
\ref{sect:stochBP_genRules}). Equation \eqref{eq:price} can be derived by 
successive application of the product rule for integrals; we provide the proofs 
for these identities in appendix \ref{app:gaussDerivProofs}. 

Equations \eqref{eq:bonnet} and \eqref{eq:price} are especially interesting 
since they allow for unbiased gradient estimates by using a 
small number of samples from $q$. 
%they allow for computations to be performed locally in the
%computational graph of the model, illustrated in figure 
%\ref{figure:introModel}(c). 
Assume that both the mean $\vmu$ and covariance matrix $\vC$ depend on 
a parameter vector $\vtheta$. We are now able to write a general rule for 
Gaussian gradient computation by combining equations \eqref{eq:bonnet} 
and \eqref{eq:price} and using the 
chain rule:
\vspace{-1mm}
\begin{equation}
\!\!\!\nabla_{\!\tiny{\vtheta}}\E_{\! \tiny{\N\!\left(\vmu, \vC\right)} }\! \left [ f(\vxi) \right ] \!=\! 
\E_{\! \tiny{\N\!\left(\vmu, \vC\right)} } \!\!\left [\! \mathbf{g}\!^\top\! \frac{\partial 
\vmu}{\partial \vtheta}\! +\! \tfrac{1}{2}\! \Tr\! \left(\!\mathbf{H} 
\frac{\partial \vC}{\partial \vtheta} \!\right) \!\right ] \label{eq:GBP}
\end{equation}
where $\vg$ and $\vH$ are the gradient and the Hessian of the function 
$f(\vxi)$, respectively. Equation \eqref{eq:GBP} can be interpreted as a modified 
backpropagation rule for Gaussian distributions that takes into account 
the gradients through the mean $\vmu$ \textit{and} covariance $\vC$. This  
reduces to the 
standard backpropagation rule when $\vC$ is constant. Unfortunately this 
rule requires knowledge of the Hessian 
matrix of $f(\vxi)$, which has an algorithmic complexity $O(K^3)$. For inference in DLGMs, we later introduce an unbiased though higher 
variance estimator that requires only quadratic complexity.
\vspace{-3mm}
\subsection{Generalised Backpropagation Rules}
\label{sect:stochBP_genRules}
%We can also derive back-propagation rules for $q$-distributions other than the Gaussian. Such rules can be derived in two ways: 
We describe two approaches to derive general backpropagation rules for non-Gaussian $q$-distributions.

\textbf{Using the product rule for integrals.}
For many exponential family distributions, it is possible to find a function 
$B(\vxi; \vtheta)$ to ensure that
\vspace{-2mm}
\begin{align}
\nabla_{\tiny{\vtheta}} \E_{\tiny{p(\vxi | \vtheta )}} [f(\vxi)] \!=\!\! =  -\E_{\tiny{p (\vxi | 
\vtheta )}} [\nabla_{\tiny{\vxi}} [B (\vxi; \vtheta) f (\vxi)]].  \nonumber
\end{align}
That is, we express the gradient with respect to the parameters of $q$ as an 
expectation of gradients with respect to the random variables themselves.
%We can thus reduce the problem to searching for a suitable transformation 
%function $B(\vxi; \vtheta)$ that allows us to compute the required derivatives 
%directly. 
This approach can be used to derive rules for many 
distributions such as the Gaussian, inverse Gamma and log-Normal. 
We discuss this in more detail in appendix
\ref{app:otherStochBPrule}. 

\textbf{Using suitable co-ordinate transformations.} \\
We can also derive stochastic backpropagation rules for any distribution 
that can be written as a smooth, invertible  transformation of a standard base 
distribution. For example, any Gaussian distribution $\N(\vmu, \vC)$ can be 
obtained as a transformation of a spherical Gaussian $\vepsilon \sim 
\N(\vzero,\vI)$, using the transformation $y = \vmu + \vR \vepsilon$ and 
$\vC = \vR \vR\!^\top\!\!$. The gradient 
of the expectation with respect to $\vR$ is then:
\vspace{-2mm}
\begin{align}
\nabla_{\tiny{\vR}} \E_{\!\N\!\left(\tiny{\vmu,\vC}\right) } \left[ 
f(\vxi) \right ]  &=\nabla_{\tiny{\vR}} 
\E_{\tiny{\N(0,I)} } \left [ f(\small{\vmu + \vR \vepsilon}) 
\right ] \nonumber \\ 
 &= \E_{ \tiny{\N(0,I)} } \left [
\vepsilon  \vg^\top \right],  \label{eq:gradR}
\end{align}
where $\mathbf{g}$ is the gradient of $f$ evaluated at $\vmu + \vR \vepsilon$ and provides a lower-cost alternative to Price's theorem \eqref{eq:price}.
%; the estimator \eqref{eq:gradR} will in general have higher variance than the 
%estimator based on \eqref{eq:price}. A short analysis of the variance of 
%these estimators is discussed in section \ref{sec:relatedWork} and in 
%appendix \ref{ap:Variance}.
%This approach can be more general than the first approach using the product 
%%%rule for integrals. 
Such transformations are well known for many distributions, especially those 
with a self-similarity property or location-scale formulation, such as the 
Gaussian, Student's $t$-distribution, stable distributions, and generalised extreme value distributions.
%; discussed further discussion in 
%appendix \ref{app:otherStochBPrule}.

\textbf{Stochastic backpropagation in other contexts.}
The Gaussian gradient identities described above do not appear to be widely used. These identities have been recognised by \citet{opper2009} for variational inference in Gaussian process regression, and following this work, by \citet{gravesNIPS2011} for parameter learning in large neural networks. 
%Our approach differs from \citet{gravesNIPS2011} since we obtain, in expectation, the full Hessian rather than a diagonal approximation. In additition, the variational approximation is improved using the low-rank covariance parameterisation we describe in section \ref{sec:learning_covParam}.
Concurrently with this paper, \citet{kingma2013auto} present an alternative discussion of
stochastic backpropagation. Our approaches were developed simultaneously and provide complementary perspectives on the use and derivation of stochastic backpropagation rules. 

==> background.tex <==
\begin{figure}[t]
 \vskip 0.2in
 \begin{center}
 \centerline{\includegraphics[width=\columnwidth]{FIGURE_Intro}}
 \caption{
 The class of generative models studied in this paper.  {\bf (a)} 
 Diagram of our model.  {\bf (b)} Diagram corresponding to 
 the equivalent representation (\ref{eq:LogLike}).
 {\bf (d)}  The computational diagram indicating the connectivity of the 
 generative and recognition models during learning.}
\label{figure:introModel}
\end{center}
\vskip -0.2in
\end{figure} 

In contrast to the Helmholtz machines originally introduced in 
\citep{Dayan1995, Dayan2000} which uses discrete latent variables, we 
have adopted  Gaussian latent variables. 

This choice was motivated by Price's \citep{Price1958} and Bonnet's 
\citep{Bonnet1964} theorems that allow us to interchange the gradients of 
expectations with respect to the moments of a Gaussian distribution with 
the expectation of gradients with respect to the random variables 
\citep{Opper2009}. These properties will be used in the next section to 
compute gradients of the generative and recognition model.

We exploit these nice properties for deriving our learning scheme in the 
following section.

In addition, we would like to model data of different types, i.e. data that 
may be binary, categorical, real-valued, etc. To achieve this objective, we 
make use of the exponential family of distributions, which is an important 
family of distributions that emphasises the shared properties of many 
standard distributions, including the Binomial, Poisson, Gamma, Beta, 
Multinomial, and Gaussian distributions \cite{book:bickel2001}. The 
exponential family of distributions allows us to provide a singular 
discussion of the inferential properties associated with members of the 
family and thus, to develop a modelling framework generalised to all 
members of the family.

In the exponential family of distributions, the conditional probability of 
some observed data vector $\vis$ 
given parameter value $\boldsymbol{\eta}$ takes the following form:
\begin{align}
\label{eq:exponFam}
 p(\vis | \boldsymbol{\eta}) &= \exp \{ s(\vis)^\top \boldsymbol{\eta} 
 + 
 h(\vis) - g(\boldsymbol{\eta}) \},
\end{align}
where $s(\vis)$ are the sufficient statistics, $\boldsymbol{\eta}$ is a 
vector of natural parameters, $h(\vis_n)$ is a function of the data and 
$g(\boldsymbol{\eta})$ is the cumulant or log-partition function. 
For convenience, we shall represent a variable $\vis$ that is drawn from 
an exponential family distribution using the notation: $\vis\sim 
\Expon{\boldsymbol{\eta}}$, with natural parameters 
$\boldsymbol{\eta}$. 

As an example, consider binary data, for which an appropriate data 
distribution is the Bernoulli distribution. The Bernoulli distribution for a 
single component $\vis_i$ has the form: 
$p(\vis_i|\mu) = \mu^{x}(1-\mu)^{1-x}$, with $\mu$ in [0,1]. The 
exponential 
family form, using the terms in Equation (\ref{eq:exponFam}), is described 
using: $h(\vis_i) = 
0$, $\eta = \ln(\frac{\mu}{1 - \mu})$ and $g(\eta) = \ln(1 + e^{\eta})$. 

The natural parameters can be mapped to the parameter values of the 
distribution using the link function, which is the logistic sigmoid in the 
case of the Bernoulli distribution.

More specifically, we are interested in directed generative models 
with a layered structure composed of $L+1$ layers, the $L$th layer being 
the topmost one as shown in Figure~\ref{figure:introModel}{\bf (a)}, 
defined by the equations:

\begin{align}
\hid_{L} &= G_{L} \xi_{L} \label{eq:xL} \\
\hid_{l} &= T_l(\hid_{l+1}) + G_{l} \xi_{l},  \forall l =1 \ldots L-1 
\label{eq:HiddenGen} \\
\vis & \sim  \Expon{T_0(\hid_{1})},
\label{eq:Visible}
\end{align}

where $\hid_{l,i}$ is the vector of activations at layer $l$,
$\xi_{l,j}$ are independent Gaussian random variables with mean 
zero and variance one, $\vis$ is the vector of observed units, 
Bern$(\vec{u})$ is a product of independent 
Bernoulli distributions with probability $p_i=\text{sigmoid}(u_i)$.

Finally $T_l$ are arbitrary maps represented by multi-layer 
perceptrons (MLPs) and $G_l$ are constant matrices. In the 
following we refer to the set of parameters in  $T_l$ and $G_l$  by 
$\theta^g$.

We adopt a weak Gaussian prior over $\theta^g$, $p(\theta^g) = 
\N(\theta| 0, \kappa)$.

This model has a likelihood function of the form

\begin{align}
p(\vis, \hid) &= p(\vis| \hid_1 ) p(\hid_L) p(\theta)
\prod_{l=1}^{L 
- 1} p_l( \hid_l | \hid_{l+1} ),\label{eq:LogLikeStandard} 
\end{align}

where $p( \hid_l | \hid_{l+1} )$ is a distribution implicitly 
defined by equation (\ref{eq:HiddenGen}) and $p(\theta)$ is a prior over 
the model's parameters. The diagram associated to this 
model is shown in Figure \ref{figure:introModel}{\bf (a)}.
 
The conditional distributions
$p_l( \hid_l | \hid_{l+1} )$ are a Gaussian distributions with mean $\mu_l 
= T_l(\hid_{l+1})$ and covariance matrix $S_l = G_l G_l^T$ due to the 
additive property of Gaussians. 

Moreover, when the maps 
$T_l$ are of the form $T_l(\hid) = A_l f(\hid) + b_l $ for some matrix 
$A_l$ and some constant vector $b_l$, 
$G_l$ is a diagonal matrix and $f$ is some 
element-wise non-linearity, Equation (\ref{eq:HiddenGen}) reduces to

\begin{align}
\hid_l &= A_l f(\hid) + b_l + C_l \xi_l,
\end{align}

and we recover the standard non-linear Gaussian belief networks 
\cite{Frey1996, 
Frey1999a}. 

Alternatively, we can interpret the variables $\hid_l$ as deterministic 
functions of the noise variables $\xi_l$.  This can be formally introduced 
as a coordinate transformation of the probability density in Equation 
(\ref{eq:LogLikeStandard}). That is, we perform a change of coordinates $
\hid_l \rightarrow \xi_{l}$. The density of the transformed variables 
$\xi$ can be expressed in terms of the density (\ref{eq:LogLikeStandard}) 
times the Jacobian of the transformation $ p(\xi)  = p(\hid(\xi)) 
|\frac{\partial \hid}{\partial \xi}| $. Since the coordinate transformation is 
linear we have $|\frac{\partial \hid}{\partial \xi}| = |G_l|$ and the density 
of $\xi$ is obtained as follows

\begin{align}
p(\xi) &= p(\hid_L)  |G_L|
\prod_{l=1}^{L - 1}  |G_l| p_l( \hid_l | \hid_{l+1} ) \nonumber  \\
&=  \prod_{l=1}^{L} |G_l| |S_l|^{-\frac{1}{2}}  \N( \xi_l ) \nonumber \\
&=  \prod_{l=1}^{L}  |G_l| |G_l G_l^T|^{-\frac{1}{2}} \N( \xi_l ) \nonumber 
\\
 &= \prod_{l=1}^{L} \N( \xi_l ), 
\end{align}
where $\N(\xi)$ is a Gaussian with mean zero and covariance equal 
to 
the identity matrix. 

Finally the joint density $p(\vis,\xi,\theta)$ can be written as 

\begin{align}
p(\vis,\xi) &= p(\vis| \hid_1( \xi_{1 \ldots L} ) ) p(\theta) 
\prod_{l=1}^{L} 
\N( \xi_l ). \label{eq:LogLike}
\end{align}

The diagram associated to this 
representation is shown in Figure \ref{figure:introModel}{\bf (b)}. 


The likelihood in Equation (\ref{eq:LogLike}) has the interesting property 
that its gradient with respect to $\xi$ backpropagates from the visible 
neurons to the last hidden layer. That is, it takes into account the 
\emph{entire network}. This is to contrast with purely local methods such 
as the wake-sleep and the mean-field algorithms which requires 
several iterations to allow the information to flow from the visible units to 
the top layers.

Moreover, this representation makes it explicit that the generative model 
works by applying a highly non-linear transformation to a spherical 
Gaussian distribution $\N(\xi)$ such that the transformed distribution tries 
to match the empirical distribution.
